A simple and versatile topology optimization formulation for flexure synthesis

High-tech equipment critically relies on flexures for precise manipulation and measurement. Through elastic deformation, flexures offer extreme position repeatability within a limited range of motion in their degrees of freedom, while constraining motion in the degrees of constraint. Topology optimization proves a prospective tool for the design of short-stroke flexures, providing maximum design freedom and allowing for application-specific requirements. State-of-the-art topology optimization formulations for flexure synthesis are subject to challenges like ease of use, versatility, implementation complexity, and computational cost, leaving a generally accepted formulation absent. This study proposes a novel topology optimization formulation for the synthesis of short-stroke flexures uniquely based on strain energy measures under prescribed displacement scenarios. The resulting self-adjoint optimization problem resembles great similarity to classic compliance minimization and inherits similar implementation simplicity, computational efficiency, and convergence properties. Numerical examples demonstrate the versatility in flexure types and the extendability of additional design requirements. The provided source code encourages the formulation to be explored and applied in academia and industry.

==> discussion.tex <==
\begin{itemize}
	\item Comparison of our method to SOTA.
	\item Paragraph on implementation in commercial software.
	\item Rigid links are assumed rigid, how to take into account elastic interfaces?
	\item Can we turn around the DOC and DOF?
\end{itemize}

\com{section that shows all the positive things of the method: low computational cost (sensitivity analysis), number of parameters, convergence etc. Basically defending ourself from our claims. All of the material required to make those claims should be presented before this section.}


\subsection{Computational efficiency}

The proposed self-adjoint method requires a single solve per degree included.
As a result, it shows superior to the kinetostatic formulations in terms of computational efficiency.
Although harder to compare, for the flexure design problem as posed, the proposed problem formulation also shows superior.
Since the kinetoelastic formulations require a solve per master \dof, it can be highly beneficial to apply multi-point constraints to the interface \dofs, a priori to static condensation towards the mechanism system matrix.
This will decrease the number of master \dofs to the number of independent \dofs of the interface, which is generally comparable to the number of degrees.

With minor modification, one may apply a robust formulation to address stress constraints and manufacturing uncertainty simultaneously, as previously proposed by \textcite{DaSilva2019} applied on compliant mechanism design. 

==> matlabcode.tex <==
\begin{lstlisting}
%%%% A 99 LINE TOPOLOGY OPTIMIZATION OF FLEXURES CODE BASED ON TOP71.M %%%%
function flexure(nelx,nely,x0,penal,rmin,A,B,Cmax)
	lA = length(A); mA = zeros(lA,3);
	lB = length(B); mB = zeros(lB,3);
	C = ["TY", "TX", "RZ"];
	for i=1:lA
		mA(i,:) = strcmp(C,A(i));
	end
	for i=1:lB
		mB(i,:) = strcmp(C,B(i));
	end
	mA = max(mA,[],1); mB = max(mB,[],1);
	nA = mA == 1;
	nB = mB == 1;
	D = find(max([mA; mB]));
	nRHS = length(D);
	assert(lA >= 1 & lA <= 2,'set A too small/big');
	assert(lB >= 1 & lB <= 2, 'set B too small/big');
	assert(nRHS >= 2 & nRHS <=3, 'incorect no of rhs');
	%% MATERIAL PROPERTIES
	E0 = 1;
	Emin = 1e-6;
	nu = 0.3;
	%% PREPARE FINITE ELEMENT ANALYSIS
	A11 = [12  3 -6 -3;  3 12  3  0; -6  3 12 -3; -3  0 -3 12];
	A12 = [-6 -3  0  3; -3 -6 -3 -6;  0 -3 -6  3;  3 -6  3 -6];
	B11 = [-4  3 -2  9;  3 -4 -9  4; -2 -9 -4 -3;  9  4 -3 -4];
	B12 = [ 2 -3  4 -9; -3  2  9 -2;  4  9  2  3; -9 -2  3  2];
	KE = 1/(1-nu^2)/24*([A11 A12;A12' A11]+nu*[B11 B12;B12' B11]);
	nodenrs = reshape(1:(1+nelx)*(1+nely),1+nely,1+nelx);
	edofVec = reshape(2*nodenrs(1:end-1,1:end-1)+1,nelx*nely,1);
	edofMat = repmat(edofVec,1,8)+repmat([0 1 2*nely+[2 3 0 1] -2 -1],nelx*nely,1);
	iK = reshape(kron(edofMat,ones(8,1))',64*nelx*nely,1);
	jK = reshape(kron(edofMat,ones(1,8))',64*nelx*nely,1);
	% DEFINE LOADS AND SUPPORTS (FLEXURE)
	ndy = 2*(nely+1);
	ndof = ndy*(nelx+1);
	U = zeros(ndof,3);
	U(2:ndy:end, 1) = 1; % TY
	U(1:ndy:end, 2:3) = 1; % TX, RZ
	U(2:ndy:end, 3) = linspace(1,-1,nelx+1); % RZ
	top = union(1:ndy:ndof,2:ndy:ndof);
	bottom = union((ndy-1):ndy:ndof,ndy:ndy:ndof);
	fixeddofs = union(top,bottom);
	alldofs = 1:ndof;
	freedofs = setdiff(alldofs,fixeddofs);
	%% PREPARE FILTER
	[dy,dx] = meshgrid(-ceil(rmin)+1:ceil(rmin)-1,-ceil(rmin)+1:ceil(rmin)-1);
	h = max(0,rmin-sqrt(dx.^2+dy.^2));
	Hs = conv2(ones(nely,nelx),h,'same');
	%% INITIALIZE ITERATION
	loop = 0;
	change = 1;
	m = 1;
	n = nelx*nely;
	x = x0*ones(n,1);
	xold1 = x;
	xold2 = x;
	low = zeros(n,1);
	upp = ones(n,1);
	dc = zeros(nely,nelx,3);
	alpha = [1 1 1];
	%% START ITERATION
	while change > 0.1
		loop = loop + 1;
		x = reshape(x,nely,nelx);
		x = (x + flip(x,1))/2;
		x = (x + flip(x,2))/2;
		xPhys = conv2(reshape(x,nely,nelx),h,'same')./Hs;
		%% FE-ANALYSIS
		sK = reshape(KE(:)*(Emin+xPhys(:)'.^penal*(E0-Emin)),64*nelx*nely,1);
		K = sparse(iK,jK,sK); K = (K+K')/2;
		U(freedofs,:) = -K(freedofs,freedofs)\(K(freedofs,fixeddofs)*U(fixeddofs,:));
		Compliance = sum(U.*(K*U));
		if loop == 1
			alpha = 1./Compliance;
		end
		for i = 1:nRHS
			X = U(:,D(i));
			ce = reshape(sum((X(edofMat)*KE).*X(edofMat),2),nely,nelx);
			dc(:,:,D(i)) = penal*(E0-Emin)*xPhys.^(penal-1).*ce;
			dc(:,:,D(i)) = conv2(dc(:,:,D(i))./Hs,h,'same');
			dc(:,:,D(i)) = (dc(:,:,D(i)) + flip(dc(:,:,D(i)),2))/2;
			dc(:,:,D(i)) = (dc(:,:,D(i)) + flip(dc(:,:,D(i)),1))/2;
		end
		%% OBJECTIVE FUNCTION AND SENSITIVITY ANALYSIS
		f = -sum(alpha(nA).*Compliance(nA));
		df = -sum(alpha(nA).*reshape(dc(:,:,nA),n,lA),2);
		g = alpha(nB).*Compliance(nB)./Cmax - 1;
		dg = alpha(nB).*reshape(dc(:,:,nB),n,lB)./Cmax;
		%% MMA UPDATE OF DESIGN VARIABLES AND PHYSICAL DENSITIES
		[xnew,~,~,~,~,~,~,~,~,low,upp] = mmasub(lB,n,loop,x(:),zeros(n,1),ones(n,1),xold1,xold2,...
		f,df,zeros(n,1),g',dg',zeros(lB,n),low,upp,1,zeros(lB,1),1000*ones(lB,1),zeros(lB,1));
		change = max(abs(xnew-x(:)));
		xold2 = xold1;
		xold1 = x(:);
		x = xnew;
		%% PRINT RESULTS
		fprintf(' It.:%3i Obj.:%4.1f, ch.:%3.2f',loop,-f,change);
		fprintf(' Con.:%4.3f',g); fprintf('\n');
		%% PLOT DENSITIES
		colormap(gray); imagesc(1-xPhys); caxis([0 1]); axis equal; axis off; drawnow;
	end
end
\end{lstlisting}


==> ror.tex <==
\paragraph{Parametrization and finite elements}
To optimize the topology each finite element $i$ is assigned a design variable $x_i \in \mathbb{R}$, which allows for local control of the material properties \autocite{Bendsoe2004}.

\paragraph{Filter}
To eliminate modelling artefacts the design variable field $\mathbf{x}$ is generally blurred as to obtain the filtered field $\tilde{\mathbf{x}}$ using a linear filtering operation with radius $r$, see \textit{e.g.} \textcite{Bruns2001}. 

\paragraph{Interpolation}
\com{Should be RAMP.}
The Young's modulus of an element is related to the filtered design variable via a composite rule.
Without loss of generality, we apply the commonly used modified Solid Isotropic Material with Penalization (SIMP) interpolation function \autocite{Sigmund2007}, that is
\begin{equation}
E_i\left[x_i\right] = \underline{E} + \left(\overline{E}-\underline{E}\right)\tilde{x}_i^p,
\end{equation}
with $\underline{E}$ and $\overline{E}$ the Young's moduli of void and solid, respectively, $p$ the penalization parameter.
%The system stiffness matrix can now be assembled as
%\begin{equation}
%\mathbf{K} = \Aop^N_{i=1} E_i \mathbf{K}^0,
%\end{equation}
%with $\Aop$ the assembly operator and $\mathbf{K}^0$ the constant element stiffness matrix.

\paragraph{Normalisation}
Without loss of generality, we opt for relating the strain energy of load case $i$ to its strain energy at the first optimization iteration, that is
\begin{equation}
\label{eq:alpha}
\alpha_i^{\{k\}}: = \frac{\mathcal{E}_i^{\{k\}}}{\mathcal{E}_i^{\{0\}}}
\end{equation}
with $k$ the optimization iteration counter. 
Note that, as a result of \cref{eq:alpha}, the normalized strain energy $\alpha$ is a dimensionless positive scalar value by definition and $\alpha_i^{\{0\}} = 1$ for all $i$. 
As a result of this normalisation, the magnitude of the prescribed displacements becomes irrelevant, as well as the difference in strain energy between different load cases a priori to the optimization.

\paragraph{Multi-objective}
Without loss of generality, we opt for a smooth minimum function as the objective \autocite{Ma1994}, that is 
\begin{equation}
f\left[\mathcal{E}_i\right] := -\frac{1}{\sum_i^{a} \frac{1}{\alpha_i\left[\mathcal{E}_i\right]}},
\end{equation}
with $a$ the number of load cases in $\mathbb{A}$.
As a result of this function, the relative strain energy which is the smallest has the greatest contribution to the objective function.
Note the triviality of this function for $a = 1$. One might, in addition, add weight factors to the individual strain energy measures to control relative significance.

\paragraph{Sensitivities}
\com{What to mention about sensitivities, there is so little to mention.}

\paragraph{Optimizer}
The design variables are iteratively updated by solving the resulting gradient-based inequality-constrained nonlinear optimization problem we apply a sequential approximate optimization scheme, as is common in the topology optimization field. To be more specific, we use the method of moving asymptotes by \textcite{Svanberg1998}. The resulting convex sub-problems are solved using a primal-dual interior point method.

\paragraph{Code}
\com{Change this section!}\\
This work is enriched with a MATLAB code, that also provides the possibility to replicate the results. 
The code can be called via \texttt{flexure(gi, gj, gjbar)}\footnote{Corresponding MATLAB code is provided in the Appendix}.  
Here, \texttt{gi} indicates the entries of set $\mathbb{A}$, \texttt{gj} the entries in set $\mathbb{B}$ and \texttt{gjbar} a list of maximum allowable normalized strain energies for the load-cases in set $\mathbb{B}$. 

\begin{table*}
	\centering
	\begin{tabular}{c|l|l|l|r}
		\toprule
		Symbol & Description & Value & Unit & Reference\\
		\midrule
		$\underline{E}$ & Young's modulus void & \SI{1.0e-6}{} & \si{\pascal}& \\
		$\overline{E}$ & Young's modulus solid & \SI{1.0}{} & \si{\pascal}& \textcite{Andreassen2011}\\
		$\nu$ & Poisson ratio & \SI{0.3}{}&- & \textcite{Andreassen2011}\\
		$p$ & SIMP penalty & \SI{3.0}{} & -&\textcite{Sigmund2007}\\
		$r$ & filter radius & \SI{2.0}{} & \text{no. of elements}&\textcite{Bruns2001}\\
		\bottomrule
	\end{tabular}
	\caption{Constants.}
\end{table*}



\subsection{Pareto fronts}
\com{One pareto front for changing constraint value as shown in \cref{fig:pareto}. Note: this figure is by no means final.}

\begin{figure*}
	\centering
	\includegraphics[width=0.9\textwidth]{figs/pareto}
	\caption{Pareto front, parameter sweep over constraint value.}
	\label{fig:pareto}
\end{figure*}

\subsection{Mesh refinement}
A clear difference is visible between primitive and complex flexures upon mesh refinement, see \cref{fig:paretotyrz,fig:paretotxty}.
\begin{figure*}
	\centering
	\includegraphics[width=0.9\textwidth]{figs/paretotyrz}
	\caption{Primitive flexure.}
	\label{fig:paretotyrz}
\end{figure*}

\begin{figure*}
	\centering
	\includegraphics[width=0.9\textwidth]{figs/paretotxty}
	\caption{Complex flexure.}
	\label{fig:paretotxty}
\end{figure*}



